Multi-label Transformer for Action Unit Detection

Action Unit (AU) Detection is the branch of affective computing that aims at recognizing unitary facial muscular movements. It is key to unlock unbiased computational face representations and has therefore aroused great interest in the past few years. One of the main obstacles toward building efficient deep learning based AU detection system is the lack of wide facial image databases annotated by AU experts. In that extent the ABAW challenge paves the way toward better AU detection as it involves a 2M frames AU annotated dataset. In this paper, we present our submission to the ABAW3 challenge. In a nutshell, we applied a multi-label detection transformer that leverage multi-head attention to learn which part of the face image is the most relevant to predict each AU.

==> sections/temporality.tex <==
\subsubsection{Enforcing temporal consistency in predictions}
We used a moving mean to smooth predictions across frames.
% The ABAW3 challenge is based on videos, \textit{i.e.} on continuous frame sequences. Furthermore, Action Units (AUs) are segment-level events as opposed to frame-level events, \textit{i.e.} activation of a specific AU (or lack of activation thereof) usually lasts for at least a couple of frames. While such temporal structure is hard to enforce with the previous frame-level framework, it can be modelled through a second neural network that takes as inputs the $s$ consecutive predictions of our multi-label transformer. 


%We denote $p_\tau \in [0;1]^{s\times T}$ the predictions from frame $\tau$ to $\tau+s$ (logits of the multi-label transformer). We define our temporal consistency operator as a function $f \rightarrow $.


%Inspired by previous work on temporal analysis \cite{lea2016temporal}, we use a 1D convolution over the $s$ dimension with fully-connected layers on top of it. For the sake of comparison, we also implemented cross-frame smoothing with 1d convolutions only and fully-connected layers only. 

%In order to compare the different models and set the parameter $s$, we trained the model with a noise on the labels $y$. Let $M^{(t)}$ be the confusion matrix associated with task $t$. 
%We tested several values for $s$ ranging from $20$ (about half a second of video) to $100$ (about 3 seconds of video).
